Model-Based Real-Time Motion Tracking using Dynamical Inverse Kinematics on SO(3)

This paper contributes towards the development of motion tracking algorithms for time-critical applications, proposing an infrastructure for solving dynamically the inverse kinematics of highly articulate systems such as humans. We present a method based on the integration of differential kinematics using distance measurement on SO(3) for which the convergence is proved using Lyapunov analysis. An experimental scenario, where the motion of a human subject is tracked in static and dynamic configurations, is used to validate the inverse kinematics method performance on human and humanoid models. Moreover, the method is tested on a human-humanoid retargeting scenario, verifying the usability of the computed solution for real-time robotics applications. Our approach is evaluated both in terms of accuracy and computational load, and compared to iterative optimization algorithms.

==> sections/back-up-notes.tex <==
\yeshisays{Kourosh and I were discussing to update this section a bit to give a bit more clarity on the problem we are talking about in the paper:
\begin{itemize}
    \item DONE: The general topic and the motivation of the paper is about inverse-kinematics of articulated models of high dimension i.e high number of links and joints like in the case of humans or humanoid models
    \item DONE: Did not present the idea of a 7DoF exactly. Present the inverse-kinematics problem with possibly a 7 DoF manipulator explaining the redundancy and then talk about more complicated articulated models like humans or humanoid robots
    \item Literature Review: The main quantities an IK problem takes as input is link frame quantities i.e frame pose with respect to the inertial frame and frame velocity with respect to the inertial frame. The two main sensor modalities to acquire input data for an IK problem are
        \begin{itemize}
            \item Computer vision based techniques: That gets the link frame quantities using vision techniques
            \item Inertial Measurements Units: That gets the link frame quantities using some sensor fusion techniques
        \end{itemize}
    Kourosh please try to see if you can find some relavant literature review.
\end{itemize}}

==> sections/optimization_based.tex <==

\section{Instantaneous Optimization Methods}
\label{section:optimization_based}
% the following optimization problem:
% \begin{subequations}\label{otimization_problem}
% \begin{align}
% & \underset{q(t),\nu(t)}{\text{minimize}}
% & & E(q(t), \nu(t), \Tilde{x}(t), \Tilde{\mathrm{v}}(t)) \\
% & \text{subject to}
% & & q_{\text{min}} \leq q(t) \leq q_{\text{max}} \\
% & & & \nu_{\text{min}} \leq \nu(t) \leq \nu_{\text{max}}
% \end{align}
% \end{subequations}
% where $E(.) \in \mathbb{R}$ is the \textit{error function} that depends on some distance measurements between the given configuration state ($q(t)$, $\nu(t)$), and the targets ($\Tilde{x}(t)$, $\Tilde{\mathrm{v}}(t)$).
% %
% \newline

% From Equation \eqref{velocity_target_equation}, it is possible to notice that the velocity $\nu(t)$ is linear with respect to task space velocity targets $\Tilde{\mathrm{v}}(t)$. The optimization problem \eqref{otimization_problem} can be then decompose into a linear optimization and a nonlinear optimization problem:
The instantaneous optimization methods are those methods that solve the inverse kinematics at each time-step $t_k$ trough non-linear programming. The inverse kinematics \textit{Problem 1} can be formulated as the stack of a linear optimization problem for the velocity $\nu(t_k)$, and a non-linear optimization for the configuration $q(t_k)$:
\begin{subequations}\label{linear_nonlinear_optimization}
\begin{align}
\label{linear_optimization}
& \underset{\nu(t_k)}{\text{minimize}}
& & dist_{\mathrm{v}}((q(t_k), \nu(t_k)), {\mathrm{v}}(t_k)) \\
& \text{subject to}
& & C\nu(t_k) \leq d \\
\label{nonlinear_optimization}
& & & \underset{q(t_k)}{\text{minimize}} & & dist_{x}(q(t_k), {x}(t_k)) \\
& & & \text{subject to} 
& & A q(t_k) \leq b
\end{align}
\end{subequations}
where $dist_x(.,.) \in \mathbb{R}$ is a measurement of the distance between the configuration state $q(t_k)$ and the target link pose ${x}$, and $dist_{\mathrm{v}}(.,.) \in \mathbb{R}$ is the measurement of the distance between the target link velocities ${\mathrm{v}}(t_k)$ and the configuration state ($q(t_k)$, $\nu(t_k)$).
%
\newline

Two different approaches for formulating and solving the nonlinear optimization problem \eqref{nonlinear_optimization} are presented in \ref{whole_body_nonlinear_optimization} and \ref{pairwised_nonlinear_optimization}. The solution of the linear optimization problem \eqref{linear_optimization}, also known as \textit{inverse differential kinematics}, is then discussed in \ref{inverse_velocity_kinematics}. The \textit{instantaneous optimization} methods do not consider the evolution of the state in time except for initializing the solver with the previous result $q^{(0)}(t_k)=q(t_{k-1})$, while the first time step is initialized with a zero configuration $q^{(0)}(t_0) = (I_{3 \times 3}, 0)$. The time dependency $(t_k)$ will be then omitted till the end of the current section. 

\subsection{Whole-Body Optimization} \label{whole_body_nonlinear_optimization}
In whole-body optimization we measure the distance between each target and the pose of the corresponding frame obtained via forward kinematics mapping $h(q)$. The position distance is measured as euclidean distance and will be indicated as $d^{p}:\mathbb{R}^3 \times \mathbb{R}^3 \to \mathbb{R}^3$, while the orientation distance is $d^{o}$ and can be measured alternatively using Euler angles ($d^o:SO(3) \times SO(3) \to \mathbb{R}^3$) or quaternion representation ($d^o:SO(3) \times SO(3) \to \mathbb{R}^4$). All the distances are collected in a single \textit{residuals vector} $r$ defined as follow:
\begin{equation}\label{residual_vector}
r(h(q),{x}) := \begin{bmatrix} d^{p}(h^{p}_{\mathcal{P}_1}(q),\prescript{\mathcal{I}}{}{{p}}_{\mathcal{P}_1}) \\\ \vdots \\\ d^{p}(h^{p}_{\mathcal{P}_{n_p}}(q),\prescript{\mathcal{I}}{}{{p}}_{\mathcal{P}_{n_p}}) \\\ d^{o}(h^{o}_{\mathcal{O}_1}(q),\prescript{\mathcal{I}}{}{{R}}_{\mathcal{O}_1}) \\\ \vdots \\\ d^{o}(h^{o}_{\mathcal{O}_{n_o}}(q),\prescript{\mathcal{I}}{}{{R}}_{\mathcal{O}_{n_o}}) \end{bmatrix}
\end{equation}
%

Defining the \textit{pose error} as the squared norm of the residual vector $r$, the optimization problem for the whole-body configuration assumes the following form:
\begin{equation}\label{wholebosy_optimization_problem}
\begin{aligned}
& \underset{q}{\text{minimize}}
& & r(h(q),{x})^T K_r r(h(q),{x}) \\
& \text{subject to}
& & Aq(t) \leq b
\end{aligned}
\end{equation}
where $K_r$ is a weight matrix that matches the unit measurements of position and orientation distances, and eventually assigns a weight to each of the target.
The algorithms for solving nonlinear optimization will not be discussed in details, since it goes beyond the purpose of the paper, for a more detailed explanation please refer to the available methods in literature\cite{ruszczynski2006}\cite{bertsekas1997}. Most of the algorithms are based on the approximation of the nonlinear system by a linear one\cite{barnes1965}\cite{fletcher1968}, and solve the problem iteratively.

\subsection{Pair-Wised Optimization} \label{pairwised_nonlinear_optimization}
For highly articulated models, and in presence of multiple targets, the method presented in \ref{whole_body_nonlinear_optimization} has to deal with high dimensional matrices that can drastically increase the computational time as shown in section \ref{results:optimization_based}. A possible solution consists in parallelizing the processing by dividing the model into multiple subsystems and to solve the problem for each subsystem independently.
%
\newline

Consider the case in which subsystems are defined by separating the model in correspondence of each target and for the \textit{base frame} both position and orientation targets are given, as in Figure \ref{fig:pairwised}. Under those conditions, the pose of the \textit{base frame} can be obtained directly by using its target position and orientation, and the joints configuration $s$ of each subsystem can be obtained by solving an optimization problem for a single relative distance measurement:
\begin{subequations}\label{reduced_orientation_optimization}
\begin{align}
&r_{\mathcal{C}\mathcal{D}}(s_{\mathcal{C}\mathcal{D}},\prescript{\mathcal{I}}{}{{p}}_{\mathcal{C}},\prescript{\mathcal{I}}{}{{p}}_{\mathcal{D}}):= d^{p}(^{\mathcal{C}}h^{p}_{\mathcal{D}}(s_{\mathcal{C},\mathcal{D}}), \prescript{\mathcal{C}}{}{{p}}_{\mathcal{D}}) \\
&r_{\mathcal{C}\mathcal{D}}(s_{\mathcal{C}\mathcal{D}},\prescript{\mathcal{I}}{}{{R}}_{\mathcal{C}},\prescript{\mathcal{I}}{}{{R}}_{\mathcal{D}}):= d^{o}(^{\mathcal{C}}h^{o}_{\mathcal{D}}(s_{\mathcal{C},\mathcal{D}}), ^{\mathcal{C}}{R}_{\mathcal{D}})
\end{align}
\end{subequations}
where $s_{\mathcal{C}\mathcal{D}} \in \mathbb{R}^{n_{\mathcal{C}\mathcal{D}}}$ is the joint configuration for the subsystem, $n_{\mathcal{C}\mathcal{D}}<n$ is the number of joints in the subsystem, and $^{\mathcal{C}}h^{p}_{\mathcal{D}}(.)$ and $^{\mathcal{C}}h^{o}_{\mathcal{D}}(.)$ are the geometrical forward kinematics mapping for the frame $\mathcal{D}$ with respect to $\mathcal{C}$. The optimization problem for each subsystem is then defined as follow:
\begin{equation}\label{subsystem_optimization_problem}
\begin{aligned}
& \underset{s_{\mathcal{C}\mathcal{D}}}{\text{minimize}}
& & {r_{\mathcal{C}\mathcal{D}}}^T K_{r_{\mathcal{C}\mathcal{D}}} r_{\mathcal{C}\mathcal{D}} \\
& \text{subject to}
& & A_{\mathcal{C}\mathcal{D}} s_{\mathcal{C}\mathcal{D}} \leq b_{\mathcal{C}\mathcal{D}} 
\end{aligned}
\end{equation}
where $A_{\mathcal{C}\mathcal{D}}$ and $b_{\mathcal{C}\mathcal{D}}$ are two parameters that take into account the constraints of the subsystem.
The solution of the problem \eqref{subsystem_optimization_problem} is analogous to the solution of the whole-body optimization problem \eqref{wholebosy_optimization_problem} presented in \ref{whole_body_nonlinear_optimization}. Though, it can be observed that the size of the residual vector $r_{\mathcal{C}\mathcal{D}}$ and the optimization variable $s_{\mathcal{C}\mathcal{D}}$ are always lower than the size of $r$ and $q$.

\begin{figure}[h]
\centering
  \includegraphics[width=0.90\columnwidth]{figs/pairwised.png}
\caption{A floating base model with eight links ($\{1\}$,$\cdots$,$\{8\}$), four orientation targets ($\prescript{\mathcal{I}}{}{{R}}_{\mathcal{B}}$, $\prescript{\mathcal{I}}{}{{R}}_{\mathcal{C}}$, $\prescript{\mathcal{I}}{}{{R}}_{\mathcal{D}}$, $\prescript{\mathcal{I}}{}{{R}}_{\mathcal{E}}$) and a single position target ($\prescript{\mathcal{I}}{}{{p}}_{\mathcal{B}}$), can be divided into three subsystems with a pair of orientation targets each.}
\label{fig:pairwised}
\end{figure}


% \subsection{Optimization-Based Methods} \label{optimization_based_methods}
% A general formulation of the optimization problem for solving the inverse kinematics is the following.
% %
% \newline
% The distance measurement can be represented by a position distance function $d^{\ell}:\mathbb{R}^3 \times \mathbb{R}^3 \to \mathbb{R}^3$ and an orientation distance function $d^a:SO(3) \times SO(3) \to \mathbb{R}^3$.
% The common approach for solving non-linear optimization is to approximate the system by a linear one, and solve the problem iteratively\cite{barnes1965}\cite{fletcher1968}. For sake of clarity, we consider first the case where there are no limit for the state configuration $q$, and a single position $\prescript{\mathcal{I}}{}{\Tilde{p}}_\mathcal{A}$ and orientation $\prescript{\mathcal{I}}{}{\Tilde{R}}_\mathcal{A}$ target are given for the same frame $\mathcal{A}$ with Jacobian $J(q)$. The solution is based on the definition of a residual vector $r=r(q) \in \mathbb{R}^6$ encoding the distance between a given configuration and the target position and orientation:
% \begin{equation}\label{residuals}
% r := \begin{bmatrix} d^{\ell}(h^{p}_\mathcal{A}(q),\prescript{\mathcal{I}}{}{\Tilde{p}}_\mathcal{A}) \\ d^a(h^{o}_\mathcal{A}(q),\prescript{\mathcal{I}}{}{\Tilde{R}}_\mathcal{A}) \end{bmatrix}
% \end{equation}
% Recalling that the Jacobian matrix can be defined as:
% \begin{equation}\label{jacobian_residual}
% \begin{aligned}
% & [J(q)]_{j,i}=\frac{\partial r_j}{\partial q_i} 
% &\begin{aligned} \forall & i =1,\ldots,(n+6) \\
% \forall & j=1,\ldots,6
% \end{aligned}
% \end{aligned}
% \end{equation}
% We can write the first term Taylor series expansion of $r(q)$ as:
% \begin{equation}\label{residual_taylor_expansion}
% \begin{aligned}
% &r(q + \delta q) &\approx \ &r(q) + \begin{bmatrix} \frac{\partial r_1}{\partial q_1} & \ldots & \frac{\partial r_1}{\partial q_{n+6}} \\ \vdots & \ddots & \vdots \\ \frac{\partial r_6}{\partial q_1} & \ldots & \frac{\partial r_6}{\partial q_{n+6}} \end{bmatrix} \delta q \\
% \\
% & &\approx \ &r(q) + J(q) \delta q
% \end{aligned}
% \end{equation}
% where $\delta q \in \mathbb{R}^{n+6}$ is an infinitesimal state space variation.

% The minimization of the residuals is then achieved by imposing the first order Taylor series \eqref{residual_taylor_expansion} equal to zero, and proceding iteratively until a stopping condition is met:
% \begin{subequations}\label{iterative_solution}
% \begin{align}\label{linear_solution}
% & r(q^{(k)}) + J(q^{(k)})\Delta q^{(k)} = 0 \\
% \label{update_state}
% & q^{(k+1)} = q^{(k)} + \Delta q^{(k)}
% \end{align}
% \end{subequations}
% Most of the algorithms for solving inverse kinematics as an optimization problem are based on this approach, and differ in the definition of the residuals or in the strategy for solving \eqref{linear_solution} to get $\Delta q^{(k)}$. The classic approach is the use of a generalized inverse\cite{rao1972}\cite{buss2004} of the Jacobian matrix:
% \begin{equation}\label{generalized_inverse}
% \Delta q^{(k)} = -J(q^{(k)})^{\dagger} r(q^{(k)})
% \end{equation}
% where $J(q^{(k)})^{\dagger} \in \mathbb{R}^{(n+6) \times 6}$ is the generalized inverse of the Jacobian $J(q^{(k)})$.
% %
% \newline

% In case there is a generic number $n_p$ of position targets and $n_o$ of orientation targets, the solver presented in \eqref{iterative_solution} is still valid by properly defining the residual vector $r(q)$ and the Jacobian $J(q)$ as:
% \begin{subequations}\label{general_residual_jacobian}
% \begin{align}\label{general_jacobian}
% & J(q) := \begin{bmatrix} J^{\ell}_{\mathcal{P}_1}(q) \\ \vdots \\ J^{\ell}_{\mathcal{P}_{n_p}}(q) \\ J^{a}_{\mathcal{O}_1}(q) \\ \vdots \\ J^{a}_{\mathcal{O}_{n_o}}(q) \end{bmatrix} \in \mathbb{R}^{(3n_p + 3n_o)}\times\mathbb{R}^{n+6} \\
% \label{general_residual}
% & r(q) := \begin{bmatrix} d^{\ell}(h^{p}_{\mathcal{P}_1}(q),\prescript{\mathcal{I}}{}{\Tilde{p}}_{\mathcal{P}_1}) \\\ \vdots \\\ d^{\ell}(h^{p}_{\mathcal{P}_{n_p}}(q),\prescript{\mathcal{I}}{}{\Tilde{p}}_{\mathcal{P}_{n_p}}) \\\ d^{a}(h^{o}_{\mathcal{O}_1}(q),\prescript{\mathcal{I}}{}{\Tilde{R}}_{\mathcal{O}_1}) \\\ \vdots \\\ d^{a}(h^{o}_{\mathcal{O}_{n_o}}(q),\prescript{\mathcal{I}}{}{\Tilde{R}}_{\mathcal{O}_{n_o}}) \end{bmatrix} \in \mathbb{R}^{(3n_p + 3n_o)}
% \end{align}
% \end{subequations}
% The Equation \eqref{general_residual} can be written in a compact form as:
% \begin{equation}\label{compact_residual}
% r(q) = d(h(q), \Tilde{x})
% \end{equation}
% where $d:\mathbb{R}^{3n_p} \times SO(3)^{n_o} \times \mathbb{R}^{3n_p} \times SO(3)^{n_o} \to \mathbb{R}^{3n_p+3n_o}$ is the aggregate distance function for all the targets, $h:\mathbb{R}^{n+6} \to \mathbb{R}^{3n_p} \times SO(3)^{n_o}$ is the aggregate forward kinematics function for all the target frames, and $\Tilde{x} \in \mathbb{R}^{3n_p} \times SO(3)^{n_o}$ is a vector collecting all the position and orientation targets.
% %
% \newline

% Recent approaches make also use of Quadratic Programming (QP) optimization in order to solve \eqref{linear_solution}, which make possible to enforce state configuration limits $q_{\text{min}}$ and $q_{\text{max}}$ by adding linear constraints\cite{Kanoun2011}. A possible formulation can be the following:
% \begin{equation}\label{otimization_problem}
% \begin{aligned}
% & \Delta q^{(k)} = 
% & &  \underset{\Delta q}{\argmin} \left\lVert r(q^{(k)}) + J(q^{(k)})\Delta q  \right\rVert + \left\lVert \lambda \Delta q \right\rVert \\
% & \text{subject to}
% & &  \\
% & & & G \Delta q \leq h \\
% \end{aligned}
% \end{equation}
% where the operator $\left\lVert . \right\rVert$ indicates the squared norm of a vector, $\lambda \in \mathbb{R}$ is a regularization term used to handle kinematics singularities, and $G$ and $h$ are two parameters used for limits avoidance that depend on $q^{(k-1)}$, $q_{\text{min}}$ and $q_{\text{max}}$.
